An Empirical Characterization of Outages and Incidents in Public Services for Large Language Models

People and businesses increasingly rely on public LLM services, such as ChatGPT, DALLE, and Claude. Understanding their outages, and particularly measuring their failure-recovery processes, is becoming a stringent problem. However, only limited studies exist in this emerging area. Addressing this problem, in this work we conduct an empirical characterization of outages and failure-recovery in public LLM services. We collect and prepare datasets for 8 commonly used LLM services across 3 major LLM providers, including market-leads OpenAI and Anthropic. We conduct a detailed analysis of failure recovery statistical properties, temporal patterns, co-occurrence, and the impact range of outage-causing incidents. We make over 10 observations, among which: (1) Failures in OpenAI's ChatGPT take longer to resolve but occur less frequently than those in Anthropic's Claude;(2) OpenAI and Anthropic service failures exhibit strong weekly and monthly periodicity; and (3) OpenAI services offer better failure-isolation than Anthropic services. Our research explains LLM failure characteristics and thus enables optimization in building and using LLM systems. FAIR data and code are publicly available on https://zenodo.org/records/14018219 and https://github.com/atlarge-research/llm-service-analysis.

==> sections/Page-budget.tex <==
\section{Plan}

\begin{figure*}[h]
  \centering
  \includegraphics[width=\linewidth]{plot/page-budget-10pages.drawio.pdf}
  \caption{Page budget.}
  \label{fig:page-budget}
  
\end{figure*}


==> sections/_6-Application-Impact-Analysis.tex <==
\section{Application-Impact Analysis}
\label{sec:analysis:appimpact}


\textbf{Notes: For new classes of applications: (1) What will be their pattern of failure, if leveraging ChatGPT or similar services? (2) Will their availability and reliability be better or worse of, relatively to running classic apps on existing datasets in existing datacenters? In other words, is your application going to fail even more when using ChatGPT (so, not only we get data that may be less credible, but also worse dependability)?}

See also Section VI in 
Alexandru Iosup, Nezih Yigitbasi, Dick H.J. Epema (2011)
On the Performance Variability of Production Cloud Services.
CCGRID 2011: 104-113. \url{https://atlarge-research.com/pdfs/2011-iosup-performance.pdf}

\textbf{ADD: two LLM Applications}


\subsection{ML Training based on ChatGPT}
\label{sec:analysis:appimpact:ml}

We assume that a new generation of applications will emerge that conduct ML training not on real-world, existing datasets, but on inputs elicited (continuously or frequently) from OpenAI --- they run on synthetically generated but realistic data produced with services such as ChatGPT or directly through API calls.

Q: How would the availability and/or performance of such services be impacted by the availability and reliability of ChatGPT services?


\subsection{Scientific Computing based on ChatGPT}
\label{sec:analysis:appimpact:scientific}




\subsection{(if time) Web Services based on ChatGPT}
\label{sec:analysis:appimpact:web}
...
- Rubis or Rubos benchmarks but with data generated by ChatGPT




